Leveraging Retrieval-Augmented Generation and Large Language Models to Predict SERCA-Binding Protein Fragments from Cardiac Proteomics Data

Large language models (LLMs) have shown promise in various natural language processing tasks, including their application to proteomics data to classify protein fragments. In this study, we curated a limited mass spectrometry dataset with 1000s of protein fragments, consisting of proteins that appear to be attached to the endoplasmic reticulum in cardiac cells, of which a fraction was cloned and characterized for their impact on SERCA, an ER calcium pump. With this limited dataset, we sought to determine whether LLMs could correctly predict whether a new protein fragment could bind SERCA, based only on its sequence and a few biophysical characteristics, such as hydrophobicity, determined from that sequence. To do so, we generated random sequences based on cloned fragments, embedded the fragments into a retrieval augmented generation (RAG) database to group them by similarity, then fine-tuned large language model (LLM) prompts to predict whether a novel sequence could bind SERCA. We benchmarked this approach using multiple open-source LLMs, namely the Meta/llama series, and embedding functions commonly available on the Huggingface repository. We then assessed the generalizability of this approach in classifying novel protein fragments from mass spectrometry that were not initially cloned for functional characterization. By further tuning the prompt to account for motifs, such as ER retention sequences, we improved the classification accuracy by and identified several proteins predicted to localize to the endoplasmic reticulum and bind SERCA, including Ribosomal Protein L2 and selenoprotein S. Although our results were based on proteomics data from cardiac cells, our approach demonstrates the potential of LLMs in identifying novel protein interactions and functions with very limited proteomic data.

==> definitions.tex <==
%%
%%
%%
%% NOTE: We want to maek this general, so that we cna copy/paste to multiple 
%% projects (grants, papers) etc 
%%
%%
%%
\newcommand{\rev}{\reversemarginpar}
\newcommand{\nor}{\par\normalmarginpar}
\newcommand{\pnote}[1]{\mnote{PKH:#1}}
%\newcommand{\bcnote}[1]{\mnote{\textcolor{blue}{BC:#1}}}
%\newcommand{\bsnote}[1]{\mnote{\textcolor{magenta}{BS: #1}}}
%\newcommand{\kinote}[1]{\mnote{\textcolor{blue}{KI:#1}}}
\newcommand{\xfnote}[1]{\mnote{\textcolor{blue}{XF:#1}}}
\newcommand{\eknote}[1]{\mnote{\textcolor{orange}{EK:#1}}}
\newcommand{\bwnote}[1]{\mnote{\textcolor{magenta}{BW:#1}}}
\newcommand{\mamnote}[1]{\mnote{\textcolor{purple}{Muqsith:#1}}}
\newcommand{\adnote}[1]{\mnote{AD:#1}}
\newcommand\addrefn[1]{\addref(#1)}
\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}
\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}


\newcommand\etal{\textit{et al}}          
\newcommand\textbt[1]{\textit{\textbf{#1}}}
\newcommand\lbi{\begin{packed_item}}
\newcommand\lei{\end{packed_item}}
\newcommand\lbn{\begin{packed_enum}}
\newcommand\len{\end{packed_enum}}
\newcommand\mytag[1]{\textbf{(#1.)}} % formats subfigure labels
\newcommand{\fig}{Fig.~\ref}
\newcommand\sfig[1]{(\textit{See } \fig{#1})}
\newcommand{\sect}{Sect.~\ref}
\newcommand\ssect[1]{(\textit{see} \secn{#1} )}
\newcommand{\tbl}{Table~\ref}
\newcommand\stbl[1]{(\textit{see} \tbl{#1} )}
\newcommand\addref{\textcolor{red}{ADD REF}}

\newcommand{\eqn}{Eq.~\ref}
\newcommand{\eqns}{Eqs.~\ref}
\newcommand{\chap}{Chapter~\ref}
\newcommand{\chaps}{Chapters~\ref}
\newcommand{\app}{Appendix~\ref}


\newcommand{\uM}{\textmu M} % or use SIunitx
\renewcommand{\um}{\textmu m}  


\newcommand{\DONE}{\textcolor{green}{ Done }}
\newcommand{\INPROGRESS}{\textcolor{blue}{ In progress }}
\newcommand{\POSTPONE}{\textcolor{yellow}{ Postpone }}
\newcommand{\NOTDONE}{\TODO}
\newcommand{\TODO}{\textcolor{red}{ To Do }}
\newcommand{\CANCEL}{\textcolor{red}{ Cancel }}
\newcommand{\mynote}[1]{\textcolor{red}{ #1 }}
\newcommand{\verify}{\mynote{verify}}
\newcommand{\bennote}[1]{\textcolor{blue}{#1}}
\newcommand{\expnote}[1]{\textbf{\textcolor{green}{#1}}}
% This enables us to more directly include source/etc in the 
% figures 
\newcommand{\codeline}[1]{\lstinline|#1|}
\newcommand{\figsquick}[5]
{
\newpage
\begin{figure}[ht]
\begin{center}
\includegraphics[width=#5]{#1}
\end{center}
\caption{
% PRINT FIGURE REFERENCE
\mynote{(figshort:#2)}
% PRINT CAPTION 
#3\label{figshort:#2}.
% PRINT DATA LOCATION 
\mynote{This figure was generated using the following notebook and dataset:}
\lstinline|#4|
}
\end{figure}
\clearpage 
\newpage
}


\newcommand{\figshort}[4]
{
  \figsquick{#1}{#2}{#3}{#4}
  {3in}
}
\newcommand{\figbig}[4]
{
  \figsquick{#1}{#2}{#3}{#4}
  {6in}
}


\newcommand{\camk}{CaMK}
\newcommand{\PKA}{[PKA]}
\newcommand{\LS}{Li-Smith}
%\renewcommand{\um}{uM}

%% right wrap
\newcommand{\FP}{Fokker\-Plank}
\newcommand{\SE}{Smoluchowski equation}
\newcommand{\rde}{Reaction-diffusion equation}
%\newcommand{\st}{single tubule}
\newcommand{\vcycle}{v$_{cycle}$}
\newcommand{\kdcasr}{K$_{d,SR}$}
\newcommand{\kd}{K$_d$}
\newcommand{\catwo}{Ca$^{2+}$}
\newcommand{\mgtwo}{Mg$^{2+}$}
\newcommand{\nap}{Na$^{+}$}
\newcommand{\kp}{K$^{+}$}
\newcommand{\caconc}{[Ca$^{2+}$]}
\newcommand{\koff}{k$_{off}$}
\newcommand{\kon}{k$_{on}$}
\newcommand{\konl}{k$_{on,luminal}$}
\newcommand{\fluo}{Fluo-3}
\newcommand{\BAR}{$\beta$-adrenergic}
\newcommand{\uplb}{uPLB}
\newcommand{\pplb}{pPLB}
\newcommand{\PDE}{partial differential equation}
\newcommand{\Kp}{$K_{P}$}
\newcommand{\SLN}{sarcolipin}
\newcommand{\rdf}{radial distribution function} 
%%% Added by Ben 
\newcommand{\tlr}{TLR4}
\newcommand{\ilob}{IL-$1\beta$}
\newcommand{\ilt}{IL-10}
\newacronym{bdnf}{BDNF}{brain derived neurotrophic factor}
\newcommand{\bdnf}{\gls{bdnf}}
\newacronym{tnf}{TNF$\alpha$}{tumor necrosis factor alpha}
\newcommand{\tnf}{\gls{tnf}}
\newcommand{\tnfa}{\tnf}
%\newcommand{\mg}{microglia}
\newcommand{\vitro}{\textit{in vitro}}
\newcommand{\vivo}{\textit{in vivo}}
\newcommand{\situ}{\textit{in situ}}
\newcommand{\nf}{NF-$\kappa B$}
\newcommand{\ifn}{INF-$\gamma$}
\newcommand{\ptxs}{$P2X7$}
\newcommand{\ptxf}{$P2X4$}
\newcommand{\cati}{$[$\catwo$]_{i}$}
\newcommand{\cato}{$[$\catwo$]_{e}$}
\newcommand{\cate}{$[$\catwo$]_{ER}$}
\newcommand{\micromole}{$\mu M$}
\newcommand{\ab}{A$\beta$}
%% G protein
\newcommand{\gaq}{$G_{\alpha q}$}
\newcommand{\gel}{$G_{11}$}
\newcommand{\gio}{$G_{i/o}$}
\newcommand{\gi}{$G_{i}$}
\newcommand{\go}{$G_{o}$}
\newcommand{\gb}{$G_{\beta}$}
\renewcommand{\gg}{$G_{\gamma}$}

\newcommand{\csection}[1]{
  \vspace{-5pt}
  \section{#1}
  \vspace{-5pt}
}
\newcommand{\csubsection}[1]{
%  \vspace{-5pt}
  \subsection*{#1}
%  \vspace{-5pt}
}
\newcommand{\csubsubsection}[1]{
%  \vspace{-5pt}
  \subsubsection*{#1}
%  \vspace{-5pt}
}
\newcommand{\vmax}{$V_{max}$}
\newcommand{\dgelec}{$\Delta G_{elec}$}
\newcommand\sone{S100A1}
\newcommand\bpv{$\beta$-PV} 
\newcommand{\bas}{$\beta$-adrenergic stimulation}
\newcommand{\fenics}{FEniCS}

% #### ACRONYMS
\newacronym{plc}{PLC}{Phospholipase C}
\newcommand\plc{\gls{plc}}
\newacronym{pkc}{PKC}{Protein kinase C}
\newcommand\pkc{\gls{pkc}}
\newacronym{dg}{DAG}{Diacylglycerol}
\newcommand\dg{\gls{dg}}

\newacronym[description={Ca2+/calmodulin-dependent protein kinase II}]
{camkii}{CaMKII}{Ca2+/calmodulin-dependent protein kinase II}
\newacronym[description={Protein kinase A}]
{PKA}{PKA}{Protein kinase A}
\newacronym[description={gain-of-function}]
{GOF}{GOF}{gain-of-function}
\newacronym[description={loss-of-function}]
{LOF}{LOF}{loss-of-function}
\newacronym[description={Ryanodine receptor}]
{ryr}{RyR}{ryanodine receptor}
\newacronym[description={root mean squared fluctuations}]
{RMSF}{RMSF}{root mean squared fluctuations}
\newacronym[description={root mean squared deviations}]
{RMSD}{RMSD}{root mean squared deviations}
\newacronym[description={nuclear magnetic resonance}]
{NMR}{NMR}{nuclear magnetic resonance}
\newacronym[description={heart failure}]
{HF}{HF}{heart failure}
\newacronym[description={knock-out}]
{KO}{KO}{knock-out}
\newacronym[description={G-protein coupled receptor}]
{GPCR}{GPCR}{G-protein coupled receptor}
\newacronym[description={non-junctional sarcoplasmic reticulum}]
{NSR}{NSR}{non-junctional sarcoplasmic reticulum}
\newacronym[description={sub-sarcolemmal space}]
{SSL}{SSL}{sub-sarcolemmal space}
\newacronym[description={junctional sarcoplasmic reticulum}]
{JSR}{JSR}{junctional sarcoplasmic reticulum}
\newacronym[description={Cardiac ventricular myocyte}]
{CVM}{CVM}{cardiac ventricular myocyte}
\newacronym[description={principal components analysis}]
{PCA}{PCA}{principal components analysis}
\newacronym[description={Brownian dynamics}]
{BD}{BD}{Brownian dynamics}
\newacronym[description={thermodynamic integration}]
{TI}{TI}{thermodynamic integration}
\newacronym[description={replica exchange molecular dynamics}]
{REMD}{REMD}{replica exchange molecular dynamics}
\newacronym[description={molecular dynamics}]
{MD}{MD}{molecular dynamics}
\newacronym[description={accelerated molecular dynamics}]
{AMD}{AMD}{accelerated molecular dynamics}
\newacronym[description={phospholamban}]
{PLB}{PLB}{phospholamban}
\newacronym[description={Diabetic cardiac myopathy}]
{DCM}{DCM}{diabetic cardiac myopathy}
\newacronym[description={Congestive heart failure}]
{CHF}{CHF}{congestive heart failure}
\newacronym[description={Ligand-binding domain}]
{LBD}{LBD}{ligand-binding domain}
\newacronym{SB}{SB}{Shannon-Bers}
\newacronym{SBM}{SBM}{Shannon-Bers-Morroti }
\newacronym{hf}{HF}{heart failure}
\newacronym[plural=DADs]{dad}{DAD}{delayed after-depolarization}
\newacronym{ucd}{UCD}{Type II diabetes UCD model}
\newcommand\ucd{\gls{ucd}}
\newacronym{apd}{APD}{action potential duration}
\newcommand\apd{\gls{apd}}
\newacronym{soce}{$SOCE$}{store operated calcium entry}
\newcommand\soce{\gls{soce}}

\newacronym{hip}{HIP}{human amylin transgenic}
\newcommand\hip{\gls{hip}}
\newacronym{amy}{+Amylin}{acute amylin-exposed mice}
\newcommand\amy{\gls{amy}}
\newacronym{SR}{SR}{sarcoplasmic reticulum}
\newcommand\SR{\gls{SR}}
\newacronym{er}{ER}{endoplasmic reticulum}
\newcommand\er{\gls{er}}
\newacronym{SL}{SL}{sarcolemma}
\newcommand\SL{\gls{SL}}
\newacronym{ecc}{ECC}{excitation-contraction coupling}
\newacronym{ap}{AP}{action potential}
\newcommand\ap{\gls{ap}}
\newacronym{tnc}{TnC}{Troponin C}
\newcommand\tnc{\gls{tnc}}
\newacronym{atp}{ATP}{adenosine triphosphate}
\newcommand\atp{\gls{atp}}
\newacronym{adp}{ADP}{adenosine diphosphate}
\newcommand\adp{\gls{adp}}
\newacronym{amp}{AMP}{adenosine monophosphate}
\newcommand\amp{\gls{amp}}
\newacronym{cam}{CaM}{calmodulin}
\newcommand\cam{\gls{cam}}
\newacronym{ncx}{NCX}{sodium/calcium exchanger}
\newcommand\ncx{\gls{ncx}}
\newacronym{nka}{NKA}{Na/K atpase}
\newcommand\nka{\gls{nka}}
\newacronym{ptyt}{$P2Y12$}{P2Y12 receptor}
\newcommand\ptyt{\gls{ptyt}}
\newacronym{ptyo}{P2Y1}{P2Y1 receptor}
\newcommand\ptyo{\gls{ptyo}}
\newacronym{pty}{$P2Y$}{P2Y receptor}
\newcommand\pty{\gls{pty}}
\newacronym{ptx}{$P2X$}{P2X receptor}
\newcommand\ptx{\gls{ptx}}
\newacronym{lcc}{LCC}{L-type Ca$^{2+}$ channel}
\newcommand\lcc{\gls{lcc}}
\newacronym{gpcr}{GPCR}{G protein coupled receptor}
\newcommand\gpcr{\gls{gpcr}}
\newacronym{nfat}{NFAT}{nuclear factor of activated T-cells}
\newcommand\nfat{\gls{nfat}}

\newacronym{fret}{FRET}{Foerster resonance energy transfer}
\newcommand\fret{\gls{fret}}

\newacronym{ipt}{$IP_3$}{Inositol trisphosphate}
\newcommand\ipt{\gls{ipt}}

\newacronym{ipr}{$IP_{3}R$}{$IP_{3}R$ receptor}
\newcommand\ipr{\gls{ipr}}

\newacronym{orai}{$ORAI$}{Calcium release-activated calcium channel protein}
\newcommand\orai{\gls{orai}}
\newacronym{stim}{$STIM1$}{Stromal interaction molecule 1}
\newcommand\stim{\gls{stim}}

\newacronym{mlck}{MLCK}{myosin light chain kinase}
\newcommand\mlck{\gls{mlck}}

\newacronym{ppi}{PPI}{protein-protein interaction}
\newcommand\ppi{\gls{ppi}}

\newacronym{pik}{PI3K}{phosphoinositide 3-kinase}
\newcommand\pik{\gls{pik}}
\newacronym{pakt}{$p$Akt}{phosphorylated Akt}
\newcommand\pakt{\gls{pakt}}
\newacronym{ent}{ENT}{ectonucleotidase}
\newcommand\ent{\gls{ent}}


\newacronym{serca}{SERCA}{Sarcoplasmic/endoplasmic reticulum calcium ATPase}
\newcommand\serca{\gls{serca}}
\newacronym[plural={transverse tubules}]{tt}{TT}{transverse tubule}
\newacronym[plural=ODEs]{ode}{ODE}{ordinary differential equations}
\newacronym[plural=CRUs]{cru}{CRU}{Ca$^{2+}$ release unit}
\newacronym{sda}{SDA}{State Decomposition Analysis}
% BEGIN: disable/enable margin notes
%-->disable margin notes
% \newcommand{\mnote}[1]{}
%-->enable margin notes
  \newcounter{mnote}
  \setcounter{mnote}{0}
  \newcommand{\mnote}[1]{\addtocounter{mnote}{1}
    \ensuremath{{}^{\bullet\arabic{mnote}}}
    \marginpar{\textit{\footnotesize\color{red}\ensuremath{\bullet\arabic{mnote}}#1}}}
  \let\oldmarginpar\marginpar
    \renewcommand\marginpar[1]{\-\oldmarginpar[\raggedleft\footnotesize
#1]%
    {\raggedright\footnotesize #1}}
% END: disable/enable margin notes

\renewcommand\tt{\gls{tt}}

\newcommand{\radko}{Rad-/-}
%\newcommand\radko{Rad$^{-/-}}
%%%
\newcommand\ODE{\gls{ode}}
\newcommand\ode{\gls{ode}}
\newcommand\cru{\gls{cru}}
\newcommand\ecc{\gls{ecc}}
\newcommand{\iclca}{$i_{\mbox{Cl(Ca)}}$}
\newcommand\icab{$i_{\mbox{CaB}}$}
\newcommand\inab{$i_{\mbox{NaB}}$}
\newcommand\inak{$i_{\mbox{NaK}}$}
\newcommand\itof{$i_{\mbox{tof}}$} % fast Cardiac transient outward potassium
\newcommand\itos{$i_{\mbox{tos}}$} % slow Cardiac transient outward potassium
\newcommand\ikr{$i_{\mbox{Kr}}$}  % - the 'rapid' delayed rectifier current /  Rapidly Activating K Current
\newcommand\iks{$i_{\mbox{Ks}}$}   % - slowly activating K+ current (not present in mouse)?
\newcommand\iki{$i_{\mbox{K1}}$}  % (I_ki) -  inward rectifier K+ current;
\newcommand\ikp{$i_{\mbox{Kp}}$} % (I_kp) - plateau potassium current;
\newcommand\ikur{$i_{\mbox{kur}}$} % slowly inactivating outward  
\newcommand\iss{$i_{\mbox{ss}}$} %  non-inactivating steady-state K+ current
\newcommand\ilcc{$i_{\mbox{CaL}}$}
\newcommand\incx{$i_{\mbox{NaCa}}$}
\newcommand\ina{$i_{\mbox{Na}}$}
\newcommand\ryr{\gls{ryr}}
\newcommand\MD{\gls{MD}}
\newcommand\md{\gls{MD}}
\newcommand\rmsd{\gls{RMSD}}
\newcommand\rmsf{\gls{RMSF}}
\newcommand\sda{\gls{sda}}
\newcommand\sbm{\gls{SBM}}
\renewcommand\sb{\gls{SB}}
\newcommand\bars{$\beta$-adrenergic stimulation} 
\newcommand\pxf{P2X4}
\newcommand\mrna{mRNA}
\newcommand\iba{Iba}   

\newcommand\ko{knock-out}   




\newcommand\muM{$\mu$M}
\newcommand\mainpt[1]{\textbf{#1}}
\newcommand\xxx{\mynote{XXX}}
\newcommand\XXX{\mynote{XXX}}

==> notes.tex <==
\newcommand{\DONE}{\textcolor{green}{ Done }}
\newcommand{\TODO}{\textcolor{red}{ Not Done }}
\newpage
\section*{Notes}
\lbi
\item Add in potential ACM journals/conferences to submit this to
  \lbi
  \item probably this https://ieeexplore.ieee.org/xpl/RecentIssue.jsp?punumber=8857
  \item IEEE Trans Comp Bio \verb!https://www.scimagojr.com/journalsearch.php?q=17971&tip=sid&clean=0!
  
  \lei
\item Resources
    \lbi
    %\item \href{https://github.com/huskeypm/llm/tree/main/sequences}{repo}
    \item \href{https://github.com/huskeypm/biochem_llm/}{repo}
    \item  \href{https://www.evernote.com/client/web?login=true#/search?query=view%3ASE%1Eproteins.csv}{evernote}
    \item embeddings were downloaded from \href{https://huggingface.co/models?other=embeddings}{link} based on the massive text embedding bookmark leaderboard 
    \lei

\mynote{Patrick? cite these } 
\begin{comment}
e5-small... there exists an arxiv reference 
https://huggingface.co/monsoon-nlp/protein-matryoshka-embeddings
? https://huggingface.co/Alibaba-NLP/gte-Qwen2-7B-instruct
https://huggingface.co/jinaai/jina-embeddings-v3
https://huggingface.co/Snowflake/snowflake-arctic-embed-xs
\end{comment}

\item Similar approach (add me) - i just reviewed a paper that did fasta embeddings for smiles (Srinivasan and Bajorath (2024).), add to 
    \lbi
    \item proteinBERT
    \item prot5 \verb!https://training.galaxyproject.org/training-material/topics/statistics/tutorials/fine_tuning_protTrans/tutorial.html!
    \item https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10815811/ <- prot structure embedding, incl llm for sequence
    \lei
\item recent nature communications paper doing the same thing for ptms published recently
\lei

\subsection{todo}
%\lbi
%\item DONE rerun against upregulated.csv (done?)
%\item DONE review images from presentation of proteins to see if anything looks good 
%\item DONE include table with append=off, rag=off, one/shot (not CoT) 
%skipCoT
%- simple hack could just comment out input/output pairs. 
%- better might be to disable all of the qualifies that are compuited (added features, rag)  
%\lei


\subsubsection{Alex}
\lbi
% \awhnote{manually, w alex} using the manual select 
\item dssp + helicity color matching
\lei

\subsubsection{Patrick}
\lbi
%\item Ask chatgpt - add hook for dssp 
\item ncludno centroid hydrophobicity verifyEq. 2
\lei
%ssh faust.luc.edu 'ssh node09 "ollama pull llama3:8b"'


\subsection{Data generation}
\subsubsection{Benchmark}
\lbi
\item \tbl{tab:f1} (from \textsc{runBenchmark.bash})
\item Follow \href{https://github.com/huskeypm/biochem_llm?tab=readme-ov-file#benchmarking}{[link]} for instructions\\
\lei
\textit{Note: all benchmarking should be done with a fairly large training database ()}

\subsubsection{control frags}
\lbi
\item validation against known (non)binders
\item \tbl{tbl:posneg} (from \textsc{runControls.bash})
\item Follow \href{https://github.com/huskeypm/biochem_llm/blob/main/README.md#miscellaneous-extended-sequences}{[controls]} for instructions
\lei
\textit{Ended up using extended fragments for this}

\subsubsection{upregulated}
\lbi
\item Continuation of predictions for MS dataset, but for those that haven't been cloned 
\item \tbl{tbl:sequence_matches} (from \textsc{runUpreg.bash})
\item Follow 
%\href{https://github.com/huskeypm/biochem_llm/blob/main/README.md#novel-sets}{[link]} 
\href{https://github.com/huskeypm/biochem_llm/blob/main/README.md#testing-novel-sets}{[link]} 
for instructions
upregulated.csv
–> testupregulated.csv using annotateData.py
\lei
\subsubsection{upregulated/membrane}
\lbi
\item get list
\begin{verbatim}
python getUniprotSubcellLoc.py 
\end{verbatim} 
\item 
\lei

 



\newpage



